Universal Hypothesis Testing with Kernels: Asymptotically Optimal Tests for Goodness of Fit

We characterize the asymptotic performance of nonparametric goodness of fit testing. The exponential decay rate of the type-II error probability is used as the asymptotic performance metric, and a test is optimal if it achieves the maximum rate subject to a constant level constraint on the type-I error probability. We show that two classes of Maximum Mean Discrepancy (MMD) based tests attain this optimality on $\mathbb R^d$, while the quadratic-time Kernel Stein Discrepancy (KSD) based tests achieve the maximum exponential decay rate under a relaxed level constraint. Under the same performance metric, we proceed to show that the quadratic-time MMD based two-sample tests are also optimal for general two-sample problems, provided that kernels are bounded continuous and characteristic. Key to our approach are Sanov's theorem from large deviation theory and the weak metrizable properties of the MMD and KSD.

==> macro_jnl.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{assumption}{Assumption}
%\newtheorem{properties}{Property}
\newtheorem{proposition}{Proposition}
%\newtheorem{conjecture}{Conjecture}
%\newtheorem{question}{Question}
%\newtheorem{criterion}{Criterion}
%\newtheorem{exercise}{Exercise}
%\newtheorem{claim}{Claim}
%\newtheorem{claim}{Claim}
\newcommand{\matplottc}[1]{               % single matlab plot twocolumn
        \unitlength .45truein
        \begin{center}
        \begin{picture}(5,4.6)(1.05,.45)
        \special{psfile=#1.ps hscale=50 vscale=50}
        \end{picture}
        \end{center}
}
\newcommand{\matplotfp}[1]{               % single matlab plot fullpage
        \unitlength .45truein
        \begin{center}
        \begin{picture}(14,16)(.8,-1)
        \special{psfile=#1.ps hscale=100 vscale=100}
        \end{picture}
        \end{center}
}
\newcommand{\matplothp}[1]{               % single matlab plot halfpage
        \unitlength .45truein
        \begin{center}  \begin{picture}(14,7.5)(-1,.55)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplothptop}[1]{               % single matlab plot halfpage
        \unitlength .45truein                % when figure is top of page
        \begin{center}  \begin{picture}(14,6.3)(-1,1.15)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplotcc}[4]{             % two axis('square') plots side by side
        \vspace{2.8in}
        \special{psfile=#1.ps voffset=-10 hoffset=-22 vscale=52 hscale=52}
        \special{psfile=/user/xu/isl/matlab/psfiles/#2.ps voffset=-10 hoffset=213 vscale=52 hscale=52}
        \hspace*{\fill}\hspace*{0.35in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.35in}#4\hspace*{\fill}
}
\newcommand{\matplottwo}[4]{             % two axis('normal') plots side by side
        \vspace{2.62in}
        \special{psfile=#1.ps voffset=-10 hoffset=-27 vscale=52 hscale=52}
        \special{psfile=#2.ps voffset=-10 hoffset=218 vscale=52 hscale=52}
        \vspace*{0.18in}
        \hspace*{\fill}\hspace*{-.05in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.65in}#4\hspace*{\fill}
}
%%
%% This is for making fancy paragraphs
%%
\def\psfancypar#1#2{\begingroup\def\par{\endgraf\endgroup\lineskiplimit=0pt}
               \setbox2=\hbox{\large\sc #2}
%              \showthe\lht2\showthe\baselineskip
               \newdimen\tmpht \tmpht \ht2 \advance\tmpht by \baselineskip
%              \showthe\tmpht
% Changed 10/2/89 rhr - t-bol -> Times-Bold for dvi2ps to dvips conversion
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
%              \showthe\ht1
               \count7=\tmpht \count8=\ht1
%  note that all this BS is necessary since TeX only does integer
%  divides and rounds all results
               \divide\count8 by 1000 \divide\count7 by \count8
%               \showthe\count7
               \tmpht=.001\tmpht\multiply\tmpht by \count7
%               \showthe\tmpht
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
               \noindent
                \hangindent1.05\wd1
               \hangafter=-2 {\hskip-\hangindent
               \lower1\ht1\hbox{\raise1.0\ht2\copy1}%
                \kern-0\wd1}\copy2\lineskiplimit=-1000pt}


\newenvironment{ap}{
\renewcommand{\thesection}{\mbox{Appendix }\Alph{section}}
\renewcommand{\thesubsection}{\Alph{section}.\arabic{subsection
}}
\renewcommand{\theequation}{\mbox{\Alph{section}.}\arabic{equation}}
}{
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\theequation}{\arabic{equation}}
}
%\def\thetabf{\hbox{\boldmath$\theta$\unboldmath}}
\def\thetabf{{\mbox{\boldmath$\theta$\unboldmath}}}
%\def\thetabf{\hbox{$\bf{\theta}$}}
\def\Upsilonbf{\hbox{\boldmath$\Upsilon$\unboldmath}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bqa}{\begin{eqnarray}}
\newcommand{\eqa}{\end{eqnarray}}
\newcommand{\bqn}{\begin{eqnarray*}}
\newcommand{\eqn}{\end{eqnarray*}}
\newcommand{\nn}{\nonumber}
\newcommand{\cl}{\centerline}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bde}{\begin{definition}}
\newcommand{\ede}{\end{definition}}
\newcommand{\bex}{\begin{example}}
\newcommand{\eex}{\end{example}}

\newcommand{\Phibf}{\mbox{${\bf \Phi}$}}
\newcommand{\Gammabf}{\mbox{${\bf \Gamma}$}}
\newcommand{\Psibf}{\mbox{${\bf \Psi}$}}

\newcommand{\thhat}{\mbox{${\hat{\thetabf}}_N$}}
\newcommand{\thbar}{\mbox{${\bar{\thetabf}}_N$}}
\newcommand{\etahat}{\mbox{${\hat{\etabf}}$}}
\newcommand{\etabf}{\mbox{${\bf\eta}$}}
\newcommand{\e}{\mbox{${\bf e}_k$}}
\newcommand{\ehat}{\mbox{$\hat{\bf e}_k$}}
\newcommand{\EWE}{\mbox{${\bf E}_s^{}{\bf WE}_s^*$}}
\newcommand{\DPD}{\mbox{$\Dbf^*\Pbf_{\bf A}^{\perp} \Dbf$}}
\newcommand{\EWEhat}{\mbox{$\hat{\bf E}_s^{}{\bf W}\hat{\bf E}_s^*$}}
\newcommand{\E}{\mbox{{\rm E}}}
\newcommand{\Es}{\mbox{${\bf E}_s^{}$}}
\newcommand{\En}{\mbox{${\bf E}_n^{}$}}
\newcommand{\Eshat}{\mbox{$\hat{\bf E}_s^{}$}}
\newcommand{\Lshat}{\mbox{$\hat {\bf \Lambda}_s^{}$}}
\newcommand{\Ls}{\mbox{$ {\bf \Lambda}_s^{}$}}
\newcommand{\Ln}{\mbox{$ {\bf \Lambda}_n^{}$}}
\newcommand{\Ltilde}{\mbox{$\widetilde {\bf \Lambda}$}}
\newcommand{\Enhat}{\mbox{$\hat{\bf E}_n^{}$}}
\newcommand{\Lnhat}{\mbox{$\hat {\bf \Lambda}_n^{}$}}
\newcommand{\Ai}{\mbox{$ ({\bf A}^*{\bf A})^{-1} $}}
\newcommand{\abf}{\mbox{${\bf a}$}}
\newcommand{\intinf}{\int_{-\infty}^{\infty}}

%Define affiliation at footnote
% Make \small be smaller (8 pt)
%\def\small{\@setsize\small{9pt}\viiipt\@viiipt\let\@listi\@listI}

\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern3pt
        \vbox{\kern3pt#1\kern3pt}\kern3pt\vrule}\hrule}}
\def\dag{{\cal y}}
\def\reals{ { {\rm  I \kern-0.15em R }  } }
\def\complex{ {\,{{\rm C} \kern-0.50em \raise0.20ex {  |}}\, }}
\def\alphabf{\hbox{\boldmath$\alpha$\unboldmath}}
\def\betabf{\hbox{\boldmath$\beta$\unboldmath}}
\def\gammabf{\hbox{\boldmath$\gamma$\unboldmath}}
\def\deltabf{\hbox{\boldmath$\delta$\unboldmath}}
\def\epsilonbf{\hbox{\boldmath$\epsilon$\unboldmath}}
\def\zetabf{\hbox{\boldmath$\zeta$\unboldmath}}
\def\etabf{\hbox{\boldmath$\eta$\unboldmath}}
\def\iotabf{\hbox{\boldmath$\iota$\unboldmath}}
\def\kappabf{\hbox{\boldmath$\kappa$\unboldmath}}
\def\lambdabf{\hbox{\boldmath$\lambda$\unboldmath}}
\def\mubf{\hbox{\boldmath$\mu$\unboldmath}}
\def\nubf{\hbox{\boldmath$\nu$\unboldmath}}
\def\xibf{\hbox{\boldmath$\xi$\unboldmath}}
\def\pibf{\hbox{\boldmath$\pi$\unboldmath}}
\def\rhobf{\hbox{\boldmath$\rho$\unboldmath}}
\def\sigmabf{\hbox{\boldmath$\sigma$\unboldmath}}
\def\taubf{\hbox{\boldmath$\tau$\unboldmath}}
\def\upsilonbf{\hbox{\boldmath$\upsilon$\unboldmath}}
\def\phibf{\hbox{\boldmath$\phi$\unboldmath}}
\def\chibf{\hbox{\boldmath$\chi$\unboldmath}}
\def\psibf{\hbox{\boldmath$\psi$\unboldmath}}
\def\omegabf{\hbox{\boldmath$\omega$\unboldmath}}
\def\Sigmabf{\hbox{$\bf \Sigma$}}
\def\Upsilonbf{\hbox{$\bf \Upsilon$}}
%\def\Phibf{\hbox{$\bf \Phi$}}
%\def\Psibf{\hbox{$\bf \Psi$}}
\def\Omegabf{\hbox{$\bf \Omega$}}
\def\Deltabf{\hbox{$\bf \Delta$}}
\def\Gammabf{\hbox{$\bf \Gamma$}}
\def\Thetabf{\hbox{$\bf \Theta$}}
\def\Lambdabf{\mbox{$ \bf \Lambda $}}
\def\Sigmabf{\mbox{$ \bf \Sigma $}}
\def\Xibf{\hbox{\bf$\Xi$}}
%\def\Pibf{{\bf$\Pi$}}
\def\Pibf{{\bf \Pi}}
\def\0bf{{\bf 0}}
\def\1bf{{\bf 1}}
\def\2bf{{\bf 2}}
\def\3bf{{\bf 3}}
\def\4bf{{\bf 4}}
\def\5bf{{\bf 5}}
\def\6bf{{\bf 6}}
\def\7bf{{\bf 7}}
\def\8bf{{\bf 8}}
\def\9bf{{\bf 9}}
\def\abf{{\bf a}}
\def\bbf{{\bf b}}
\def\cbf{{\bf c}}
\def\dbf{{\bf d}}
\def\ebf{{\bf e}}
\def\fbf{{\bf f}}
\def\gbf{{\bf g}}
\def\hbf{{\bf h}}
\def\ibf{{\bf i}}
\def\jbf{{\bf j}}
\def\kbf{{\bf k}}
\def\lbf{{\bf l}}
\def\mbf{{\bf m}}
\def\nbf{{\bf n}}
\def\obf{{\bf o}}
\def\pbf{{\bf p}}
\def\qbf{{\bf q}}
\def\rbf{{\bf r}}
\def\sbf{{\bf s}}
\def\tbf{{\bf t}}
\def\ubf{{\bf u}}
\def\vbf{{\bf v}}
\def\wbf{{\bf w}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\zbf{{\bf z}}
\def\rbf{{\bf r}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\Abf{{\bf A}}
\def\Bbf{{\bf B}}
\def\Cbf{{\bf C}}
\def\Dbf{{\bf D}}
\def\Ebf{{\bf E}}
\def\Fbf{{\bf F}}
\def\Gbf{{\bf G}}
\def\Hbf{{\bf H}}
\def\Ibf{{\bf I}}
\def\Jbf{{\bf J}}
\def\Kbf{{\bf K}}
\def\Lbf{{\bf L}}
\def\Mbf{{\bf M}}
\def\Nbf{{\bf N}}
\def\Obf{{\bf O}}
\def\Pbf{{\bf P}}
\def\Qbf{{\bf Q}}
\def\Rbf{{\bf R}}
\def\Sbf{{\bf S}}
\def\Tbf{{\bf T}}
\def\Ubf{{\bf U}}
\def\Vbf{{\bf V}}
\def\Wbf{{\bf W}}
\def\Xbf{{\bf X}}
\def\Ybf{{\bf Y}}
\def\Zbf{{\bf Z}}
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}

\def\amat{\mathcal{a}}
\def\bmat{\mathcal{b}}
\def\cmat{\mathcal{c}}
\def\dmat{\mathcal{d}}
\def\emat{\mathcal{e}}
\def\fmat{\mathcal{f}}
\def\gmat{\mathcal{g}}
\def\hmat{\mathcal{h}}
\def\imat{\mathcal{i}}
\def\jmat{\mathcal{j}}
\def\kmat{\mathcal{k}}
\def\lmat{\mathcal{l}}
\def\mmat{\mathcal{m}}
\def\nmat{\mathcal{n}}
\def\omat{\mathcal{o}}
\def\pmat{\mathcal{p}}
\def\qmat{\mathcal{q}}
\def\rmat{\mathcal{r}}
\def\smat{\mathcal{s}}
\def\tmat{\mathcal{t}}
\def\umat{\mathcal{u}}
\def\vmat{\mathcal{v}}
\def\wmat{\mathcal{w}}
\def\xmat{\mathcal{x}}
\def\tmat{\mathcal{y}}
\def\zmat{\mathcal{z}}

\def\Amat{\mathcal{A}}
\def\Bmat{\mathcal{B}}
\def\Cmat{\mathcal{C}}
\def\Dmat{\mathcal{D}}
\def\Emat{\mathcal{E}}
\def\Fmat{\mathcal{F}}
\def\Gmat{\mathcal{G}}
\def\Hmat{\mathcal{H}}
\def\Imat{\mathcal{I}}
\def\Jmat{\mathcal{J}}
\def\Kmat{\mathcal{K}}
\def\Lmat{\mathcal{L}}
\def\Mmat{\mathcal{M}}
\def\Nmat{\mathcal{N}}
\def\Omat{\mathcal{O}}
\def\Pmat{\mathcal{P}}
\def\Qmat{\mathcal{Q}}
\def\Rmat{\mathcal{R}}
\def\Smat{\mathcal{S}}
\def\Tmat{\mathcal{T}}
\def\Umat{\mathcal{U}}
\def\Vmat{\mathcal{V}}
\def\Wmat{\mathcal{W}}
\def\Xmat{\mathcal{X}}
\def\Ymat{\mathcal{Y}}
\def\Zmat{\mathcal{Z}}

%\def\be{\vskip .3cm \begin{equation}}
%\def\ee{\end{equation} \vskip .4cm \noindent}
%
\def\defeq{{\stackrel{\Delta}{=}}}
%
%\newtheorem{theorem}{Theorem}[chapter]
%\newtheorem{conjecture}{Conjecture}[chapter]
%\newtheorem{lemma}{Lemma}[chapter]
%\newtheorem{definition}{Definition}[chapter]
%\newtheorem{corollary}{Corollary}[chapter]
%\newcounter{remarknr}[chapter]
%\newenvironment{remark}{\vskip\baselineskip
%\stepcounter{remarknr}\noindent{\bf
%Remark~\theremarknr.}}{\ \hfill $\Box$ \vskip\baselineskip}
%\newcounter{examplenr}[chapter]
%\newenvironment{example}[1]{\vskip\baselineskip
%\stepcounter{examplenr}\noindent{{\bf
%Example~\thechapter.\theexamplenr}\hskip .8em #1\\}}{\ \hfill $\Box$
%\vskip\baselineskip}
\newcommand{\x}{\mbox{${\bf x}(t)$}}
\newcommand{\s}{\mbox{${\bf s}(t)$}}
\newcommand{\n}{\mbox{${\bf n}(t)$}}
\newcommand{\jj}{\mbox{${\bf j}(t)$}}
\newcommand{\R}{\mbox{$\hat {\bf R}_{N}$}}
\newcommand{\Rhat}{\mbox{$\hat {\bf R}$}}
\newcommand{\A}{\mbox{${\cal A}$}}
%\newcommand{\Ad}{\mbox{${\cal A}^d$}}
\newcommand{\D}{\mbox{${\cal D}$}}
\newcommand{\M}{\mbox{{\bf M}}}
\newcommand{\Tr}{\mbox{Tr}}
\newcommand{\pbox}{\hfill $\Box$}
\newcommand{\blankline}{\vskip\baselineskip\noindent}
\def\Rxx{\Rbf_{\ssstyle X\kern-.1em X}}
\def\rxx{\hbox{$\Rxx$}}
\def\ryy{\hbox{$\Rbf_{\ssstyle YY}$}}
\def\rxy{\hbox{$\Rbf_{\ssstyle XY}$}}\def\ryx{\hbox{$\Rbf_{\ssstyle YX}$}}
\def\rxyT{\hbox{$\Rbf_{\ssstyle XY}^*$}}\def\ryxT{\hbox{$\Rbf_{\ssstyle YX}^*$}}
\def\Rss{\Rbf_{\ssstyle SS}}
\def\rss{\mbox{$\Rss$}}
\def\Rnn{\Rbf_{\ssstyle NN}}
\def\rnn{\hbox{$\Rnn$}}
\def\rxxinv{\hbox{$\Rbf^{-1}_{\ssstyle XX}$}}
\def\Rssinv{\Rbf^{-1}_{\ssstyle SS}}
\def\rssinv{\hbox{$\Rssinv$}}
\def\rzzinv{\Rbf^{-1}_{\ssstyle ZZ}}\let\rzzi=\rzzinv
\def\hatrxx{\widehat{\Rbf}_{\ssstyle XX}}
\def\hatrzz{\widehat{\Rbf}_{\ssstyle ZZ}}
\def\hatrss{\widehat{\Rbf}_{\ssstyle SS}}
\def\phstar{{\phantom{*}}}
\let\rzzhat=\hatrzz \let\rxxhat=\hatrxx \let\Rxxhat=\rxxhat
\let\ssstyle=\scriptscriptstyle
\let\rsshat=\hatrss
% I add the following!
\def\eqorneq{=\!\!\!\! ? \,\,}
\def\ltornlt{? \!\!\!\!\! <}
\def\sN{{\ssstyle N}}
\def\sM{{\ssstyle M}}
\def\sF{{\ssstyle F}}
\def\sT{{\ssstyle T}}
\def\sH{{\ssstyle H}}
\def\sK{{\ssstyle K}}
\def\sL{{\ssstyle L}}
\def\sQ{{\ssstyle Q}}
\def\sV{{\ssstyle V}}
\def\cross{\!  \times  \!}
\def\alphat{\alpha^{(t)}}
\def\alphab{\alpha^{(b)}}
\def\betat{\beta^{(t)}}
\def\betab{\beta^{(b)}}
\def\ATbf{{\bf A_\sT}}
\def\AHbf{{\bf A_\sH}}
\def\sspan{\mbox{\it span}}
\def\eg{{\it e.g.,}}
\def\etal{{\it et al. \/}}
\def\viz{{\it viz.,\ \/}}
\def\ie{{\it i.e.,\ \/}}
\def\Kout{\setbox1=\hbox{\Huge\bf K}\hbox to
1.05\wd1{\hspace{.05\wd1}\special{
"/Times-BoldItalic findfont 25 scalefont setfont
/prKzip
{0 0 moveto (K) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prKzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prKzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (K) true charpath  stroke
 grestore
} def
dozip}}}
\def\Sout{\setbox1=\hbox{\Huge\bf S}\hbox to 1.05\wd1{\hspace{.05\wd1}\special{"
/Times-BoldItalic findfont 25 scalefont setfont
/prSzip
{0 0 moveto (S) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prSzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prSzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (S) true charpath  stroke
 grestore
} def
dozip}}}








